On the Difficulty of Defending Contrastive Learning against Backdoor Attacks

Recent studies have shown that contrastive learning, like supervised learning, is highly vulnerable to backdoor attacks wherein malicious functions are injected into target models, only to be activated by specific triggers. However, thus far it remains under-explored how contrastive backdoor attacks fundamentally differ from their supervised counterparts, which impedes the development of effective defenses against the emerging threat. This work represents a solid step toward answering this critical question. Specifically, we define TRL, a unified framework that encompasses both supervised and contrastive backdoor attacks. Through the lens of TRL, we uncover that the two types of attacks operate through distinctive mechanisms: in supervised attacks, the learning of benign and backdoor tasks tends to occur independently, while in contrastive attacks, the two tasks are deeply intertwined both in their representations and throughout their learning processes. This distinction leads to the disparate learning dynamics and feature distributions of supervised and contrastive attacks. More importantly, we reveal that the specificities of contrastive backdoor attacks entail important implications from a defense perspective: existing defenses for supervised attacks are often inadequate and not easily retrofitted to contrastive attacks. We also explore several alternative defenses and discuss their potential challenges. Our findings highlight the need for defenses tailored to the specificities of contrastive backdoor attacks, pointing to promising directions for future research.

==> backup/abstract.tex <==
\begin{abstract}
    We present \attack, a simple yet effective backdoor attacks against CL. With both empirical and analytical evidence, we show that (i) CL is highly vulnerable to backdoor attacks; (ii) the attacks against CL and supervised learning (SL) work through different mechanisms, demonstrating distinguishable patterns in terms of neuron activation and feature distributions; (iii) due to such unique characteristics, the existing defenses for SL are largely inapplicable to CL. 
\end{abstract}

==> backup/intro.tex <==

\section{Sketch}

1. what makes SSL vulnerable? (contrastive loss + data augmentation)
2. what are the implications of such unique vulnerability for defenses? 1) from data perspective, feature-inseparability (which makes defenses based on latent separability fail) 2) from model perspective, distributions of lipschitz coefficient (which makes defenses based on neuron anomaly fail)
3. what are the general implications of such vulnerability (semantic replacement?)
4. case study (gender classification + hats), more like "bias" than "attack"
5. Discuss debias method









Distillation can remove backdoor: 10 min, 10000

4. Training set: Male + Female (No Hats) + A small set Male (Wearing Hats)

Gender classification

Test Set (normal): 80\%

Test Set (Male + Wearing Hats): 78\%

Test Set (Female + Wearing Hats): 45\% - 56\%, i.e., close to random guess.


Trigger: More robust


% \begin{table*}[t]
% \centering
% \begin{tabular}{llll}
% \hline
% Method & Clean & Backdoor(Clean label) & + Clip \\ \hline

% Frequency  \cite{wang2021backdoor}    &              &       &          \\ \hline





%  BadNets \cite{gu2019badnets}  &     \begin{tabular}[c]{@{}l@{}}$D_p = \{(x_i +\delta, t)\}$, $x_i$ from any class\\ $D = D_c \cup D_p$\end{tabular}            &   $\gL   =  \E_{x,y \in \gD}\, \ell(h(x; \theta), y) $            &     $h(x), h' = h$         \\\hline
%  Label-consistent \cite{turner2019label}     &    \begin{tabular}[c]{@{}l@{}} find $z_1, z_2$ such that $G(z_1/z_2) \approx x_1/z_2 $ \\ 
%  $D_p = \{(G(\alpha z_1 + (1-\alpha)z_2) +\delta, y_1)\}$, $x_1$ \\
%  from target class, $x_2$ from an incorrect class \\$D = D_c \cup D_p$\end{tabular}             &      $\gL   =  \E_{x,y \in \gD}\, \ell(h(x; \theta), y) $          &   $h(x), h' = h$            \\ \hline
%  EntangledWatermark  \cite{jia2021entangled}    &    \begin{tabular}[c]{@{}l@{}}$D_p = \{(x_i +\delta, t)\}$, $x_i$ from source class\\ $D = D_c \cup D_p$\end{tabular}               &   \begin{tabular}[c]{@{}l@{}}$\gL   = \beta \E_{x,y \in \gD}\, \ell(h(x; \theta), y)$ \\$ + (1 - \beta) \gL_{SNNL}$\end{tabular}             &     $h(x), h' = h$          \\ \hline
 
%                               &                 &               &              \\
%                                           &                 &               &              \\
%       &                 &               &              \\ \hline
% \end{tabular}
% \end{table*}



\section{Introduction}


A plethora of backdoor attacks are available against supervised and contrastive learning. We reveal two fundamental mechanisms that enable backdoor attacks: 
\begin{itemize}
    \item  Trigger overfitting -- (directly) associating trigger inputs with target-class labels. 
    \item  Feature entanglement -- (indirectly) associating trigger inputs and target-class inputs in the latent space. 
\end{itemize}

In this study, we ask the following questions: 
\begin{itemize}
    \item What are their fundamental connections?
    \item Which mechanisms do the existing backdoor attacks adopt?
    \item What are their implications for defenses?
\end{itemize}


\subsection{Experimental design}

{\bf Trigger.} To exclude the influence of the trigger definition, we consider two trigger definitions: \mct{i} local, spatial-domain patching and \mct{ii} global, spectral-domain perturbation. 

{\bf Poisoning attacks.} We consider two poisoning attacks: \mct{i} target-class -- applying triggers only to target-class inputs; \mct{ii} all-class -- applying triggers to inputs from all the classes. 

\subsubsection{Effectiveness} 
Under both SL and CL settings, we show that both attacks work as expected.

\subsubsection{Incompatibility} 
We switch the attacks against SL and CL and show that they do not work any more, indicating that the two attacks work through different mechanisms.

\subsubsection{Mechanisms}
Concretely, we measure the difference of the two attacks as reflected in various model- and data-statistics, including \mct{i} the entanglement between the latent representations of trigger and target-class inputs (to show the feature-entanglement effect), \mct{ii} the distributions of Lipschitz coefficients (to show the trigger-overfitting effect). \ting{the names of the effects TBD}




\subsubsection{Spectrum of backdoor attacks}
Let $\gD$ be the poisoning data (including both clean data $\gD_c$ and poisoning data $\gD_p$) and $\gD_t$ be the data from target class $t$. Let $h$ be the the model: $h = g \circ f$ in which $f$ and $g$ represent the feature extractor and classifier respectively. 



% We may define the joint poisoning loss: 
% \begin{align}
%     \gL  = \lambda \gL_\mathsf{to} + ( 1 - \lambda) \gL_\mathsf{fe}\\
% \gL_\mathsf{to}   =  \E_{x \in \gD}\, \ell(h(x; \theta), t) \\
% \gL_\mathsf{fe}   =  \E_{x \in \gD_t}\,\Delta ( f(x; \theta), \phi_t)  
% \end{align}
Poisoning Data Generation:
$(x+\delta, y)$




Training Loss:
\begin{align}
\gL  = \alpha\beta \gL_\mathsf{back} + (1-\alpha)\beta  \gL_\mathsf{clean} + (1-\beta) \gL_\mathsf{entangle}\\
\gL_\mathsf{back}   =  \E_{x,y \in \gD_p}\, \ell(h'(x; \theta'), y) \\
\gL_\mathsf{clean}   =  \E_{x,y \in \gD_c}\, \ell(h(x; \theta), y) \\
\gL_\mathsf{entangle} = \E_{x \in \gD_p}\,\Delta ( f'(x; \theta_f), \phi_t) 
%\gF = \alpha\beta h'(x) + (1-\alpha)\beta h(x) + (1-\beta) \Delta ( f'(x; \theta), \phi_t)
\end{align}


Model Output:
\begin{align}
\gF = \alpha h'(x) + (1-\alpha) h(x)
\end{align}


% We may define the joint poisoning loss: 
% \begin{align}
%     % \gL  = \lambda \gL_\mathsf{to} + ( 1 - \lambda) \gL_\mathsf{fe}\\
% \gL   =  \E_{x \in \gD}\, \ell(\gF(x), t) \\
% %\gL_\mathsf{fe}   =  \E_{x \in \gD_t}\,\Delta ( f(x; \theta), \phi_t)  
% \end{align}



Here, $h(x;\theta)$ is the $h$'s prediction about $x$ while $f(x; \theta_f)$ is $x$'s latent representation (with a little abuse of notations, we use $\theta$ to denote the parameters of both $f$ and $h$); $\ell$ measures the prediction loss; $\Delta$ measures the similarity between $x$'s representation and the representation $\phi_t$ of target-class $t$.

We may instantiate $\Delta$ with different forms. For example, in latent backdoor, it is defined as:
\begin{equation}
    \Delta(f(x; \theta), t) = \| f(x; \theta) - \phi_t  \|^2
\end{equation}
where $\phi_t$ is instantiated as the average representation of class $t$. \ting{list other instantiations} While the concrete definitions vary, they all tend to induce the feature entanglement effect. 

BadNets \cite{gu2019badnets}: In this scenario, we train the backdoor task and clean task end-to-end. Therefore, we have $h' = h$, i.e., they have the same architectures and weights. Besides, we do not require the two tasks entangled in the feature space. So, we have $\beta = 1$.
So, the model becomes the following:

$$\gL   =  \E_{x,y \in \gD}\, \ell(h(x; \theta), y) $$
%\gF = \alpha\beta h'(x) + (1-\alpha)\beta h(x) + (1-\beta) \Delta ( f'(x; \theta), \phi_t)



\begin{table*}[t]
\begin{tabular}{cccccc}
\hline
Method & Clean Model & \begin{tabular}[c]{@{}c@{}}Backdoor Moldel\\ (Clean Label, Unclip)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Backdoor Moldel\\ (Clean Label, Clip)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Backdoor Moldel\\ (Wrong Label, Unclip)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Backdoor Moldel\\ (Wrong Label, Clip)\end{tabular} \\ \hline
  Frequency  \cite{wang2021backdoor}       &     81\% / 9.7\%        &        79\% / 12\%                                                                        &          44\% / 22\%                                                                     &                       79\% / 99\%                                                           &       66\% / 99\%                                                                        \\
  BadNets     &       --      &            --                                                                     &                 --                                                              &                79\% / 98\%                                                                 &           49\% / 79\%                                                                    \\
       &             &                                                                                 &                                                                               &                                                                                 &                                                                               \\
       &             &                                                                                 &                                                                               &                                                                                 &                                                                               \\
       &             &                                                                                 &                                                                               &                                                                                 &                                                                               \\
       &             &                                                                                 &                                                                               &                                                                                 &                                                                               \\
       &             &                                                                                 &                                                                               &                                                                                 &                                                                               \\
       &             &                                                                                 &                                                                               &                                                                                 &                                                                               \\
       &             &                                                                                 &                                                                               &                                                                                 &                                                                               \\ \hline
\end{tabular}
\end{table*}

Label-consistent: It contains two kinds of methods: latent space interpolation and adversarial perturbations. Next, we analyze them one by one \cite{turner2019label}. For latent space interpolation, the authors use WGAN to get the interpolation between the trigger example and the target class example. Similar to BadNets, we have $h' = h$ here. The difference is that it implicitly entangle the trigger inputs and the target class inputs. Then, the model becomes the following:




\begin{align}
\gL  = \beta \E_{x,y \in \gD}\, \ell(h(x; \theta), y) + (1-\beta) \gL_\mathsf{entangle}\\
\gL_\mathsf{entangle} = \E_{x \in \gD_t}\,\Delta ( f(x; \theta_f), \phi_t) 
%\gF = \alpha\beta h'(x) + (1-\alpha)\beta h(x) + (1-\beta) \Delta ( f'(x; \theta), \phi_t)
\end{align}


\begin{table*}[t]
\centering
\begin{tabular}{llll}
\hline
Method & Poisoning  Data & Training Loss & Model Output \\ \hline
 BadNets \cite{gu2019badnets}  &     \begin{tabular}[c]{@{}l@{}}$D_p = \{(x_i +\delta, t)\}$, $x_i$ from any class\\ $D = D_c \cup D_p$\end{tabular}            &   $\gL   =  \E_{x,y \in \gD}\, \ell(h(x; \theta), y) $            &     $h(x), h' = h$         \\\hline
 Label-consistent \cite{turner2019label}     &    \begin{tabular}[c]{@{}l@{}} find $z_1, z_2$ such that $G(z_1/z_2) \approx x_1/z_2 $ \\ 
 $D_p = \{(G(\alpha z_1 + (1-\alpha)z_2) +\delta, y_1)\}$, $x_1$ \\
 from target class, $x_2$ from an incorrect class \\$D = D_c \cup D_p$\end{tabular}             &      $\gL   =  \E_{x,y \in \gD}\, \ell(h(x; \theta), y) $          &   $h(x), h' = h$            \\ \hline
 EntangledWatermark  \cite{jia2021entangled}    &    \begin{tabular}[c]{@{}l@{}}$D_p = \{(x_i +\delta, t)\}$, $x_i$ from source class\\ $D = D_c \cup D_p$\end{tabular}               &   \begin{tabular}[c]{@{}l@{}}$\gL   = \beta \E_{x,y \in \gD}\, \ell(h(x; \theta), y)$ \\$ + (1 - \beta) \gL_{SNNL}$\end{tabular}             &     $h(x), h' = h$          \\ \hline
 Frequency  \cite{wang2021backdoor}    &       \begin{tabular}[c]{@{}l@{}}$D_p = \{(P(x_i), t)\}$, $x_i$ from any class\\ $D = D_c \cup D_p$\end{tabular}           &     $\gL   =  \E_{x,y \in \gD}\, \ell(h(x; \theta), y) $         &    $h(x), h' = h$           \\ \hline
 TrojanNet \cite{tang2020embarrassingly}       &     \begin{tabular}[c]{@{}l@{}}$D_p = \{x_i + \delta_j, t_j)\}$, $x_i$ from any class\\ $D = D_c \cup D_p$\end{tabular}             &   
 \begin{tabular}[c]{@{}l@{}}  $\gL  = \alpha \E_{x,y \in \gD_p}\, \ell(h'(x; \theta'), y)$ \\
+ $ (1-\alpha)\E_{x,y \in \gD_c}\, \ell(h(x; \theta), y) $
 \end{tabular}
         &   $\alpha h'(x) + (1-\alpha) h(x)   $        \\ \hline
LatentBackdoor \cite{yao2019latent}      &    \begin{tabular}[c]{@{}l@{}}$D_p = \{(x_i + \delta, y)\}$, $x_i$ from any class\\ $D = D_c \cup D_p$\end{tabular}               &        \begin{tabular}[c]{@{}l@{}}  $\gL   = \alpha \E_{x,y \in \gD}\, \ell(h(x; \theta), y)$ \\
+ $ (1-\alpha)\E_{x,y \in \gD_p} D( f(x; \theta) , \phi_t) $
 \end{tabular}        &       $h(x), h' = h$                \\ \hline
TrojanNN  \cite{liu2017trojaning}          &      \begin{tabular}[c]{@{}l@{}}$D_p = \{(x_i + \delta, t)\}$, $x_i$ is the generated \\ example that maximize the output of a\\ non-target class, $\delta$ is maximized the \\selected neurons\end{tabular}                       &     $\gL   =  \E_{x,y \in \gD_p}\, \ell(h(x; \theta), y) $           &      $h(x), h' = h$          \\ \hline
Reflection     \cite{liu2020reflection}                 &        \begin{tabular}[c]{@{}l@{}}$D_p = \{(x_i + x_r	\otimes k, y)\}$, $x_i$ from \\target class, $k$ is the convolutional \\ kernel $D = D_c \cup D_p$\end{tabular}           &       $\gL   =  \E_{x,y \in \gD_p}\, \ell(h(x; \theta), y)$       &     $h(x), h' = h$          \\ \hline
 ABE \cite{shokri2020bypassing}                         &     \begin{tabular}[c]{@{}l@{}}$D_p = \{(x_i +\delta, t)\}$, $x_i$ from any class\\ $D = D_c \cup D_p$\end{tabular}              &  
  \begin{tabular}[c]{@{}l@{}}$\gL   =  \E_{x,y \in \gD}\, \ell(h(x; \theta), y) - $\\
  $\beta \ell_{Dis}(Dis(f(x)), B(x))$ \\
$ \gL_{Dis}   = \ell_{Dis}(Dis(f(x)), B(x)) $ \\
$B(x)$ is 1 if $x \in D_p$ else 0
   \end{tabular}          &       $h(x), h' = h$            \\ \hline
 IMC \cite{pang2020tale}                                  &                 &               &              \\
                                          &                 &               &              \\
       &                 &               &              \\ \hline
\end{tabular}
\end{table*}


The entanglement is included in the poisoning process. For a poisoning input, it is generated by a generator: $x = G(\tau z_1 + (1-\tau) z_2)$, where $z_1$ is the latent representation of the target class example and  $z_2$ is that of another class example. Then, the adversary apply a trigger to the generated poisoning example and assign the target class label.


The second one is adversarial perturbations. The adversary perturb the original target class input to a wrong class. This can also be explained by the feature entanglement. After generated the adversarial example, the adversary still assign its original label.


EntangledWatermark: We have $h' = h$ here.  \cite{jia2021entangled}: 


\begin{align}
\gL  = \beta \E_{x,y \in \gD}\, \ell(h(x; \theta), y) + (1-\beta) \gL_\mathsf{entangle}\\
\gL_\mathsf{entangle} = SNNL()
\end{align}

Frequency: \cite{wang2021backdoor} The authors used the frequency trigger and assigned the poisoned example with target class label.
$$\gL   =  \E_{x,y \in \gD}\, \ell(h(x; \theta), y). $$

TrojanNet: \cite{tang2020embarrassingly} The adversary first trains a trojan neural network and inserts it into the target network. The model output can be denoted as the following:


% $$\gF  =   \alpha h'(x) + (1 - \alpha) h(x), \alpha \in (0.5, 1) \\
% \gL_\mathsf{back}   =  \E_{x,y \in \gD_p}\, \ell(h'(x; \theta'), y) \\
% \gL_\mathsf{clean}   =  \E_{x,y \in \gD_c}\, \ell(h(x; \theta), y) $$
\begin{align*}
\gF  =   \alpha h'(x) + (1 - \alpha) h(x), \alpha \in (0.5, 1)\\
\gL_\mathsf{back}   =  \E_{x,y \in \gD_p}\, \ell(h'(x; \theta'), y) \\
\gL_\mathsf{clean}   =  \E_{x,y \in \gD_c}\, \ell(h(x; \theta), y) \\
%\gF = \alpha\beta h'(x) + (1-\alpha)\beta h(x) + (1-\beta) \Delta ( f'(x; \theta), \phi_t)
\end{align*}
.

TrojanNN: 1) Trigger generation: make the selected neurons have the largest activations. 2) Training data generation. 3) Retrain the model.

The poisoning process mainly focus on date generation.

LatentBackdoor: \cite{yao2019latent}.








With empirical evaluation, we may show that by properly adjusting $\lambda$, it is possible to reformulate the existing backdoor attacks within the spectrum of backdoor attacks, with varying emphasis on either trigger overfitting or feature entanglement. We may illustrate this observation using a 2D-chart with x- an y-axes as the two effects.


\subsubsection{Implications for defenses} 
The spectrum of backdoor attacks has profound implications for defense design, such as \mct{i} many defenses either implicitly or explicitly rely on the assumption of latent separability, which does not hold for attacks based on feature entanglement. \mct{ii} it is possible to integrate both mechanisms to build more effective and evasive attacks \ting{?}


==> setup.tex <==
\section{Experimental Difference}

\subsection{Experimental Setup}

{\bf Datasets --} Our evaluation primarily uses two benchmark datasets for contrastive learning methods: CIFAR-10\mcite{cifar} consists of 60,000 32$\times$32 color images divided into 10 classes; CIFAR-100\mcite{cifar100} is similar to CIFAR-10 but includes 100 classes, each of 600 images.

{\bf CL methods --} We mainly use three representative contrastive learning methods,  SimCLR\mcite{chen:2020:simple}, BYOL\mcite{grill:2020:bootstrap}, and MoCo\mcite{he2020momentum}. 

{\bf Models --} We use an encoder with ResNet-18\mcite{resnet} as its backbone and a two-layer MLP projector to map the representations to a 128-dimensional latent space.
